Fine-tuning CLIP Text Encoders with Two-step Paraphrasing

Contrastive language-image pre-training (CLIP) models have demonstrated considerable success across various vision-language tasks, such as text-to-image retrieval, where the model is required to effectively process natural language input to produce an accurate visual output. However, current models still face limitations in dealing with linguistic variations in input queries, such as paraphrases, making it challenging to handle a broad range of user queries in real-world applications. In this study, we introduce a straightforward fine-tuning approach to enhance the representations of CLIP models for paraphrases. Our approach involves a two-step paraphrase generation process, where we automatically create two categories of paraphrases from web-scale image captions by leveraging large language models. Subsequently, we fine-tune the CLIP text encoder using these generated paraphrases while freezing the image encoder. Our resulting model, which we call ParaCLIP, exhibits significant improvements over baseline CLIP models across various tasks, including paraphrased retrieval (with rank similarity scores improved by up to 2.0% and 5.6%), Visual Genome Relation and Attribution, as well as seven semantic textual similarity tasks.

==> sections/5_analysis.tex <==
\section{Analysis}

\subsection{Comparison of Data Augmentation Methods}

\input{tables/data_augs}



\subsection{Case Study}

We manually analyzed retrieval results of baseline CLIP models and our ParaCLIP for the original queries and their paraphrased queries.
We used the queries in the paraphrased retrieval dataset, and 5K images from the validation set and 41K images from the test set.


==> sections/6_related_work.tex <==
\section{Related Work}
\label{sec:related_work}

Recent studies have raised vision-language models' limitations in understanding textual inputs such as compositional understanding~\cite{thrush2022winoground,yuksekgonul2022and}.


==> tables/data_augs.tex <==
\begin{table}[t]
\centering
\footnotesize
\begin{tabular}{lccc}
\toprule
 & \textbf{P Rtrv.} & \textbf{STS} & \textbf{Clsf.} \\
\cmidrule(lr){2-2} \cmidrule(lr){3-3} \cmidrule(lr){4-4}
\textbf{Method} & \textbf{AO@10} & \textbf{Spmn.} & \textbf{Acc} \\
\midrule
CLIP &  &  &  \\
\midrule
Unsupervised &  &  &  \\
\midrule
\multicolumn{4}{l}{\textbf{\textit{Supervised data}}} \\
MS COCO &  &  &  \\
Flickr30k (318K) &  &  &  \\
SNLI+MNLI (314K) &  &  &  \\
\midrule
\multicolumn{4}{l}{\textbf{\textit{Synthetic data (Ours)}}} \\
ChatGPT (300K) &  &  &  \\
LLaMA (300K) &  &  & \\
\bottomrule
\end{tabular}
\caption{Performance of different data augmentation methods.}
\label{tab:data_augs}
\end{table}

==> tables/loss_ablation.tex <==
\begin{table}[t]
\centering
\footnotesize
\begin{tabular}{lll|cc|cc}
\toprule
\multicolumn{3}{l|}{\textbf{Loss}} & \textbf{P Rtrv.} & \textbf{STS} & \textbf{Cls.} & \textbf{I Rtrv.} \\
\cmidrule(lr){4-4} \cmidrule(lr){5-5} \cmidrule(lr){6-6} \cmidrule(lr){7-7}
&& & \textbf{AO@10} & \textbf{Avg.} & \textbf{Acc} & \textbf{R@5} \\
\midrule
X & X & X &  &  &  \\
\midrule
L1 &  &  &  \\
L1 &  &  &  \\
L1 &  \\
L2 &  \\
L1 &  \\
\bottomrule
\end{tabular}
\caption{}
\label{tab:loss_ablation}
\end{table}

==> tables/sts_results.tex <==
\begin{table*}[t]
\centering
\footnotesize
\begin{tabular}{lcccccccc}
\toprule
\textbf{Model} \textbf{(Data)} & \textbf{STS12} & \textbf{STS13} & \textbf{STS14} & \textbf{STS15} & \multicolumn{1}{c}{\textbf{STS16}} & \textbf{STS-B} & \multicolumn{1}{c}{\textbf{SICK-R}} & \textbf{Avg.} \\
\midrule
\multicolumn{9}{l}{\textit{\textbf{OpenAI's CLIP (400M)}}} \\
No fine-tuning & 72.3 & 65.0 & 55.1 & 64.3 & 70.4 & 61.7 & 66.7 & 65.1   \\
CLIP-FT & 71.3 & 68.2 & 61.7 & 68.8 & 72.4 & 68.3 & 71.1 & 68.8 \\
Ours (step 1) & 72.6  & 66.9 & 62.0 & 68.8 & 69.5 & 68.2 & 68.3 & 68.0  \\
CLIP & 72.0 &  70.8 & 65.1 & 72.2 & 72.4 & 71.1  & 69.2 & 70.3 \\
\midrule
\multicolumn{6}{l}{\textit{\textbf{OpenCLIP (LAION-2B)}}} & \\
Ours (step 1) & 68.89 & 65.53 & 62.88 & 73.09 & 69.01 &  68.47   & 70.74  & 68.37 \\
\midrule
\multicolumn{9}{l}{\textit{\textbf{LaCLIP (LAION-400M augmented with paraphrases)}}} \\
No fine-tuning &&&&&&&& 58.8 \\
CLIP-FT & 50.1 & 64.7 & 57.8 & 69.4 & 70.2 & 60.5 & 68.1 & 63.0 \\
Our CLIP & 69.0 & 65.7 & 62.5 & 73.3 & 68.9 & 68.2 & 69.3 & 68.1 \\
Our CLIP \\
\bottomrule
\end{tabular}
\caption{Zero-shot performance of CLIP models with different fine-tuning strategies on five evaluation tasks. See the main text for details on models and metrics. ``Rtrv.'': Retrieval. ``Spmn.'': Spearman's rank correlation. ``Clsf.'': Classification.}
\label{tab:sts_results}
\end{table*}
